PuzzleGPT: Emulating Human Puzzle-Solving Ability for Time and Location Prediction

The task of predicting time and location from images is challenging and requires complex human-like puzzle-solving ability over different clues. In this work, we formalize this ability into core skills and implement them using different modules in an expert pipeline called PuzzleGPT. PuzzleGPT consists of a perceiver to identify visual clues, a reasoner to deduce prediction candidates, a combiner to combinatorially combine information from different clues, a web retriever to get external knowledge if the task can't be solved locally, and a noise filter for robustness. This results in a zero-shot, interpretable, and robust approach that records state-of-the-art performance on two datasets -- TARA and WikiTilo. PuzzleGPT outperforms large VLMs such as BLIP-2, InstructBLIP, LLaVA, and even GPT-4V, as well as automatically generated reasoning pipelines like VisProg, by at least 32% and 38%, respectively. It even rivals or surpasses finetuned models.

==> latex/tables/acc_stdacc.tex <==
\begin{table}
  \centering
  \begin{tabular}{l|cc}
    \toprule
    \textbf{Model} & \textbf{Acc$^*$ (\%)} &\textbf{Acc}  \\
    \midrule
    BLiP2           & \textit{17.41}  &    1.97     \\
    LLaVA           & 7.85   &      0.61    \\
    Video-LLaMA     & 0.00  &      0.00     \\
    GPT4o           & 16.62  &    4.88      \\
    \midrule
    PuzzleGPT            & \textbf{22.99}  &\textbf{1.76}         \\
    \bottomrule
  \end{tabular}
  \caption{Standardized accuracies on VLM baselines and our results.}
  \label{standard}
\end{table}

==> latex/tables/f1_f1beta.tex <==
\begin{table*}[t]
  \centering
  \begin{tabular}{lcccc}
    \toprule
         &    \multicolumn{2}{c}{\textbf{Time}}
         &\multicolumn{2}{c}{\textbf{Location}} \\
    \midrule
    \textbf{Model}  & \textbf{Example-F1}     & \textbf{Example-F1}$^\beta$   & \textbf{Example-F1}     &\textbf{Example-F1}$^\beta$  \\
    \midrule
    BLiP2  &  36.81 & 32.27  &  49.98   & 43.59  \\
    LLaVA    &  \textit{43.84} & \textit{43.26}   & 33.82  & 25.92  \\
    Video-LLaMA&  34.68 & 21.44  & 9.07     &  6.99 \\
    GPT-4o    &  38.50 & 21.94  &  \textit{54.81}   & \textit{47.16}  \\
    InstructBLiP& \textbf{49.56} & 36.34 & 5.13    & 4.40\\
    IdealGPT & 34.11  & 26.83  & 30.27   & 25.70 \\
    \midrule
    PuzzleGPT     &43.72   & \textbf{43.72}  &\textbf{56.11}      & \textbf{51.04} \\
    \bottomrule
  \end{tabular}
  \caption{\label{tab:tara_main_results}
   Experiments conducted on TARA. We compared our results with Generative VLMs and denoted the best performance as \textbf{bold} and the second best as \textit{italic}. We also included a comparison of the scores after adding a brevity penalty.
  }
\end{table*}


==> latex/tables/metric.tex <==
\begin{table}
  \centering
  \begin{tabular}{l|c}
    \toprule
    \textbf{Model} & \textbf{Acc$^*$ (\%)} \\
    \midrule
    CLiP            & 11.11           \\
    CLiP+           & 15.72           \\
    CLiP+Seg        & 16.46           \\
    QR-CLiP         & 19.31           \\
    \midrule
    BLiP2           & \textit{17.41}           \\
    LLaVA           & 7.85            \\
    Video-LLaMA     & 0.00            \\
    GPT4o           & 16.62           \\
    \midrule
    Ours            & \textbf{22.99}           \\
    \bottomrule
  \end{tabular}
  \caption{Standardized accuracies on VLM baselines and our results.}
  \label{standard}
\end{table}

==> latex/tables/tara_ablation.tex <==
\begin{table*}[t]
  \centering
  % \begin{adjustbox}{width=1\textwidth}
  % \small
  \begin{tabular}{lcccc}
    \toprule
         &      \multicolumn{2}{c}{\textbf{Time}}&\multicolumn{2}{c}{\textbf{Location}}\\
    \midrule
    \textbf{Ablations}       & \textbf{Example-F1}     & \textbf{Example-F1}$^\beta$   & \textbf{Example-F1}     & \textbf{Example-F1}$^\beta$ \\
    \midrule
    Base  & \textbf{43.72}   &  \textbf{43.72}   &\textbf{ 56.11}  & \textbf{51.04}\\
    -Remove Filtering  &  39.27 & 39.27     & 52.10   &  48.77  \\
    -1st Hie Only      &  42.62 &  42.62    & 50.09  & 46.68   \\
    -3rd Hie Only      &  42.72 & 42.72     & 48.63  &  45.21   \\
    -Hash Threshold=7  &  43.63 & 43.63     &  55.37  &  50.31   \\
    -Hash Threshold=3  &  43.68 & 43.68     &  55.98  &   \textit{51.04}   \\
    -Retrieval Threshold=80     & 43.61 &  43.61 &  55.62   & 50.55\\
    -Retrieval Threshold=95     & \textit{43.67} &  \textit{43.67}  &   \textit{56.07}  &   49.93   \\
    -No Retrieval      &  42.63  & 42.63    & 47.65     & 43.30  \\
    -Retrieval text-image matching   & 43.47   & 43.47    &  55.91     & 50.95  \\
    \bottomrule
  \end{tabular}
  \caption{\label{tara_ablation}
    We conducted an ablation study on TARA to evaluate the impact of each component in PuzzleGPT. Our findings show that PuzzleGPT achieves optimal performance when all components are utilized together.
  }
  % \end{adjustbox}
\end{table*}


==> latex/tables/tara_main_results.tex <==
\begin{table*}[t]
  \centering
  \begin{tabular}{l|cccccc}
    \toprule
         &    & \textbf{Time}  &  &  & \textbf{Location} & \\
    \midrule
    \textbf{Model}  &\textbf{Acc(\%) \upperarrow}            & \textbf{Example-F1}     & $\beta$      & \textbf{Acc(\%)} & \textbf{Example-F1}     & $\beta$  \\
    \midrule
    CLiP       & 0.46   &  39.90 & -     & 11.11 & 44.96    & -  \\
    CLiP+      & 1.00   &  43.09 & -     & 15.72 & 49.74    & -  \\
    CLiP+Seg   & 0.92   &  42.82 & -     & 16.46 & 50.52    & -  \\
    QR-CLiP    & 3.53   &  47.89 & -     & 19.31 & 50.96    & -  \\
    \midrule
    BLiP2      & 0.30   &  36.81 & 32.27  & 1.63  &  49.98   & 43.59  \\
    LLaVA      & 0.23   &  43.84 & \textbf{43.26}   & 0.34  & 33.82  & 25.92  \\
    Video-LLaMA &0.00   &  34.68 & 21.44   & 0.00  & 9.07     &  6.99 \\
    GPT4o      &0.30    &  38.50 & 21.94 & \textbf{4.88}  &  \textit{54.81}   & 47.16  \\
    InstructBLiP  & 0.00 & \textbf{49.56} & 36.34 & 0.07 & 5.13    & 4.40\\
    IdealGPT   & 0.27     & 34.11  & 26.83 &  1.49  & 30.27   & 25.70 \\
    \midrule
    Ours(base)       &{0.38}  &42.36   & \textit{40.84} & \textit{1.76}   &54.50      & \textit{50.37} \\
    Ours(Best)       &{0.30}  &\textit{43.86}   & 43.68 & \textit{1.76}   &\textbf{56.21}      & \textbf{50.51} \\
    \bottomrule
  \end{tabular}
  \caption{\label{tab:tara_main_results}
   Experiments conducted on TARA. We compared our results with Generative VLMs and denoted the best performance as \textbf{bold} and the second best as \textit{italic}. We also included a comparison of the scores after adding a brevity penalty.
  }
\end{table*}


==> prompts1.tex <==
\subsection{Perceiver Prompts}
\textbf{Image Summary}

\definecolor{backcolor}{rgb}{0.95,0.95,0.92}
\begin{lstlisting}[backgroundcolor = \color{backcolor}, basicstyle=\small, breaklines=true]
USER: <image>
What are the words shown in this image? 
Short Answer: ASSISTANT:
\end{lstlisting}
\textbf{Initial Guess}
\begin{lstlisting}[backgroundcolor = \color{backcolor}, basicstyle=\small, breaklines=true]
USER: <image>
What are the 3 most possible cities where this image was most likely taken in? Separate the answers with commas. 
Short Answer: ASSISTANT:
\end{lstlisting}
\textbf{Image Keywords}
\begin{verbatim}
"""
USER: <image>
Keywords of this image? Answer with the keywords 
only and separate with commas. 
Short Answer: ASSISTANT:
"""
\end{verbatim}
\textbf{Supplimentary Keywords}
\begin{verbatim}
"""
USER: <image>
What are the keywords of this image? Answer 
with the keywords only and separate with commas. 
Short Answer: ASSISTANT: 
"""
\end{verbatim}
\textbf{Date Candidate}
\begin{verbatim}
"""
USER: <image>
In what date was this image taken? 
Short Answer: ASSISTANT: 
"""
\end{verbatim}
\textbf{Check Confidence of Location}
\begin{verbatim}
"""
USER: <image>
Are you confident this image was taken in {loc}? 
Short Answer: ASSISTANT: 
"""
\end{verbatim}
\textbf{If Has Landmark}
\begin{verbatim}
"""
USER: <image>
Are you confident that this point to a specific
location such as a city, country or a continent?
Answer with yes or no. 
Short Answer: ASSISTANT: 
"""
\end{verbatim}
\textbf{Check Celebrity}
\begin{verbatim}
"""
USER: <image>
Are you confident that this person is famous?
Answer with yes or no: ASSISTANT: 
"""
\end{verbatim}
\textbf{Get Celebrity Name}
\begin{verbatim}
"""
USER: <image>
What is the name of this celebrity that you are 
most confident with? ASSISTANT: 
"""
\end{verbatim}
\subsection{Online Retriever Prompts}
\textbf{Key Words}
\begin{verbatim}
"""
"{contexts}"
"{main_text}"
Given above words and characters, please remove 
the unrecognizable words and organize the most
informative words to a clean text. Please be concise
and informative. 
Short Answer:
"""
\end{verbatim}
\subsection{Noise Filter}
\textbf{Check Location for Location Confidence}
\begin{verbatim}
"""
"{snippet}"
"{location_result}"
Given above text and location, are they pointing 
to the same location? 
Answer yes or no: '
"""
\end{verbatim}
\textbf{Get Location}
\begin{verbatim}
"""
What is the most possible city associated with 
{snippet}? Answer the location only and avoid 
any prompts. 
Short Answer:
"""
\end{verbatim}
Where snippet is the text snippet retrieved by the retriever.
\subsection{Reasoner Prompts}
\textbf{Extract Event}
\begin{verbatim}
"""
Can you conclude this text in at most 3 words 
and remove non-specific details:
"{event}"
"""
\end{verbatim}
\textbf{Convert Date Format}
\begin{verbatim}
"""
Convert the date {date_candidate} to 
yyyy-mm-dd. Answer the corresponding 
yyyy-mm-dd only. 
Short Answer:
"""
\end{verbatim}
\textbf{Check Location Validity}
\begin{verbatim}
"""
Honestly speaking, do you think "{loc}" is a 
valid city or country or continent? Answer with 
yes or no only. 
Short Answer:
"""
\end{verbatim}
\textbf{Concrete Keywords}
\begin{verbatim}
"""
"{event}"
"{keywords}"
Above texts are describing an same event. Please 
conclude the event with no more than 5 words. Keep 
your answer informative, short and concise. 
Short Answer:
"""
\end{verbatim}
\textbf{Find Events}
\begin{verbatim}
"""
"{event}"
{keywords}"
Do any of the above text contains location 
information such as city, country or continent? 
If yes, please answer that city, country or 
continent. Otherwise, answer No. 
Short Answer:
"""
\end{verbatim}
\textbf{Get Continent}
\begin{verbatim}
"""
What is the continent that {country} is located 
in? Answer with the continent only and avoid 
any prompts. 
Short Answer:
"""
\end{verbatim}
\textbf{Get Time Range}
\begin{verbatim}
"""
What is the most possible time range with {name}?
Format your answer as "start-end" and answer the
range only. 
Short Answer:
"""
\end{verbatim}
\textbf{Clean Text}
\begin{verbatim}
"""
"{contexts}"
"{main_text}"
Given above words and characters, please remove 
the unrecognizable words and organize the most 
informative words to a clean text. Please be 
concise and informative. 
Short Answer:
"""
\end{verbatim}
\textbf{Get Time Candidate}
\begin{verbatim}
"""
"{time_clue}"
Given above information, please ground a specific
year or month or date from it and answer with it 
only. If you can not find a date, answer No. 
Short Answer:
"""
\end{verbatim}
\textbf{Check Date Candidate}
\begin{verbatim}
"""
"{time_range}"
"{date_result}"
Is the time range aligned with the later date? 
Answer Yes or No only. 
Short Answer:
"""
\end{verbatim}

